Preprocessing is All You Need: Boosting the Performance of Log Parsers With a General Preprocessing Framework

Log parsing has been a long-studied area in software engineering due to its importance in identifying dynamic variables and constructing log templates. Prior work has proposed many statistic-based log parsers (e.g., Drain), which are highly efficient; they, unfortunately, met the bottleneck of parsing performance in comparison to semantic-based log parsers, which require labeling and more computational resources. Meanwhile, we noticed that previous studies mainly focused on parsing and often treated preprocessing as an ad hoc step (e.g., masking numbers). However, we argue that both preprocessing and parsing are essential for log parsers to identify dynamic variables: the lack of understanding of preprocessing may hinder the optimal use of parsers and future research. Therefore, our work studied existing log preprocessing approaches based on Loghub, a popular log parsing benchmark. We developed a general preprocessing framework with our findings and evaluated its impact on existing parsers. Our experiments show that the preprocessing framework significantly boosts the performance of four state-of-the-art statistic-based parsers. Drain, the best statistic-based parser, obtained improvements across all four parsing metrics (e.g., F1 score of template accuracy, FTA, increased by 108.9%). Compared to semantic-based parsers, it achieved a 28.3% improvement in grouping accuracy (GA), 38.1% in FGA, and an 18.6% increase in FTA. Our work pioneers log preprocessing and provides a generalizable framework to enhance log parsing.

==> sections/discussions.tex <==
\section{Discussions}
\label{sec:discussions}
As analyzed in Sec.~\ref{sec:study_results}, the combination of our preprocessing framework and the state-of-the-art log parsers has brought visible improvement in terms of parsing accuracies. However, we acknowledge that the combination still failed to overcome the performance gap between statistic and semantic-based parsers. Under the guidance of training data, deep learning models can effectively learn features of the variables and their corresponding masks. Conversely, no current statistic-based log parser analyzes the masking standards in the ground-truth templates. We stated in Sec.~\ref{sec:preprocessing_problems} that the unconventional placeholders will cause the downside of parsing accuracies (i.e., PA and FTA), even though we have accurately and precisely identified the variables. 

We also noticed that although both the preprocessing framework and semantic-based tools are highly variable-aware, the grouping accuracies (i.e., GA and FTA) gained by the latter are higher. We reason this outcome as the learning ability of language models. Semantic-based tools such as LogPPT and UniParser can infer the data-specific masking fashion based on the labels and reduce the number of wrongly masked tokens, for example, some of the package names. 

While they can have more balanced performances, the reasoning process of semantic-based tools is more difficult to maintain and explain. A precedent study points out that interpretable systems are easier to manage and debug in the long run~\cite{rudin2019stop}. We argue that labeling several log messages with templates and identifying a few system-specific variable patterns are equally time-consuming for researchers and developers. With a more precise 

==> tables/combination_performance.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{The average GA, FGA, PA, and FTA obtained by the preprocessing framework as a standalone parser (i.e., Preprocess-O), and the highest average values when combined with parsers (i.e., Combined). }
\label{tab:combination_performance}
\resizebox{0.65\columnwidth}{!}{%
\begin{tabular}{l|l|l|l|l}
\hline
                      & \textbf{GA} & \textbf{FGA} & \textbf{PA} & \textbf{FTA} \\ \hline
\textbf{Preprocess-O} & 0.681       & 0.635        & 0.590       & 0.412        \\ \hline
\textbf{Combined}     & 0.764       & 0.801        & 0.58        & 0.576        \\ \hline
\end{tabular}%
}
\end{table}

==> tables/parser_selection.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Parsers selected for the study. }
\label{tab:parser_selection}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|l}
\hline
\textbf{Type}             & \textbf{Parser}               \\ \hline
\textbf{Frequency-based}  & LFA~\cite{nagappan2010abstracting}, LogCluster~\cite{vaarandi2015logcluster}, Logram~\cite{dai2020logram}, SLCT~\cite{vaarandi2003data} \\ \hline
\textbf{Similarity-based} & LenMa~\cite{shima2016length}, LogMine~\cite{hamooni2016logmine}, LogSig~\cite{tang2011logsig}        \\ \hline
\textbf{Heuristic-based} & \begin{tabular}[c]{@{}l@{}}AEL~\cite{jiang2008abstracting}, Drain~\cite{he2017drain}, IPLoM~\cite{makanju2009clustering}, \\ MoLFI~\cite{messaoudi2018search}, SHISO~\cite{mizutani2013incremental}, Spell~\cite{du2016spell}\end{tabular} \\ \hline
\end{tabular}%
}
\end{table}


==> tables/performance_difference.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{The increment in average GA, FGA, PA, and FTA before and after the preprocessing framework refinement. A positive value indicates the value increased after the modification; a negative value suggests the value decreased due to the new preprocessing framework. }
\label{tab:performance_difference}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l|l|l}
\hline
\textbf{Metrics} &
  \textbf{AEL} &
  \textbf{Drain} &
  \textbf{IPLoM} &
  \textbf{LenMa} &
  \textbf{LFA} &
  \textbf{LogCluster} &
  \textbf{LogMine} &
  \textbf{Logram} &
  \textbf{LogSig} &
  \textbf{MoLFI} &
  \textbf{SHISO} &
  \textbf{SLCT} &
  \textbf{Spell} \\ \hline
\textbf{Average GA} &
  -6.452\% &
  -10.434\% &
  -5.175\% &
  +4.145\% &
  +3.698\% &
  +2.665\% &
  -11.717\% &
  +40.72\% &
  -5.754\% &
  +14.376\% &
  +1.025\% &
  +17.463\% &
  -19.74\% \\ \hline
\textbf{Average FGA} &
  +8.676\% &
  +7.951\% &
  -0.914\% &
  +33.333\% &
  +5.81\% &
  +15.615\% &
  +26.608\% &
  +41.304\% &
  +3.519\% &
  +36.116\% &
  +18.393\% &
  +16.209\% &
  +3.14\% \\ \hline
\textbf{Average PA} &
  +104.947\% &
  +83.601\% &
  +65.366\% &
  +323.846\% &
  +20.737\% &
  +300.806\% &
  +114.692\% &
  +228.916\% &
  +406.364\% &
  +357.292\% &
  +390.217\% &
  +110.895\% &
  +12.67\% \\ \hline
\textbf{Average FTA} &
  +122.65\% &
  +105.714\% &
  +71.779\% &
  +316.154\% &
  +49.254\% &
  +75.0\% &
  +203.03\% &
  +150.862\% &
  +553.846\% &
  +514.286\% &
  +315.079\% &
  +105.97\% &
  +21.512\% \\ \hline
\end{tabular}%
}
\end{table*}

==> tables/preprocessor_performance.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{The minimum, maximum, and average values of each metric obtained by the preprocessing framework on the 14 datasets. }
\label{tab:preprocessor_performance}
\resizebox{0.65\columnwidth}{!}{%
\begin{tabular}{l|l|l|l|l}
\hline
              & \textbf{GA} & \textbf{FGA} & \textbf{PA} & \textbf{FTA} \\ \hline
\textbf{Min.} & 0.189       & 0.114   & 0.173    & 0.044        \\ \hline
\textbf{Max.} & 1.0         & 1.0         & 0.978        & 0.714        \\ \hline
\textbf{Avg.} & 0.681       & 0.635       & 0.590        & 0.412        \\ \hline
\end{tabular}%
}
\end{table}

==> tables/refined_examples.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{An example of refined preprocessing regexes and their corresponding masks (placeholders). }
\label{tab:refined_examples}
\resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{l|l|l}
\hline
\textbf{Semantic} & \textbf{Regex} & \textbf{Mask} \\ \hline
Time &
  \textbackslash{}d\{2\}:\textbackslash{}d\{2\}:\textbackslash{}d\{2\}(,\textbackslash{}d+)? &
  \textless{}*\textgreater{}:\textless{}*\textgreater{}:\textless{}*\textgreater{} \\ \hline
IPV4 with port &
  (/|)(\textbackslash{}d+\textbackslash{}.)\{3\}\textbackslash{}d+(:\textbackslash{}d+) &
  \textless{}*\textgreater{}:\textless{}*\textgreater{} \\ \hline
Duration time &
  \textbackslash{}\textless{}?\textbackslash{}d+\textbackslash{}s?sec &
  \textless{}*\textgreater{} \\ \hline
\end{tabular}%
}
\end{table}
